Translingual Obfuscation

Program obfuscation is an important software protection technique that prevents attackers from revealing the programming logic and design of the software. We introduce translingual obfuscation, a new software obfuscation scheme which makes programs obscure by "misusing" the unique features of certain programming languages. Translingual obfuscation translates part of a program from its original language to another language which has a different programming paradigm and execution model, thus increasing program complexity and impeding reverse engineering. In this paper, we investigate the feasibility and effectiveness of translingual obfuscation with Prolog, a logic programming language. We implement translingual obfuscation in a tool called BABEL, which can selectively translate C functions into Prolog predicates. By leveraging two important features of the Prolog language, i.e., unification and backtracking, BABEL obfuscates both the data layout and control flow of C programs, making them much more difficult to reverse engineer. Our experiments show that BABEL provides effective and stealthy software obfuscation, while the cost is only modest compared to one of the most popular commercial obfuscators on the market. With BABEL, we verified the feasibility of translingual obfuscation, which we consider to be a promising new direction for software obfuscation.

==> longversion.tex <==
\renewcommand{\shortlong}[2]{#2}


==> plot/plot-dist-logscale <==
set term pdf size 6,3 font "Aerial,15"
set output "plot/dist-logscale.pdf"
set size ratio 0.6
set yrange [0.01:100]
set xrange [-1:27]
set logscale y
set datafile separator ","
set xtics border out nomirror rotate by -45 
#set xtics border out scale 0,0 nomirror rotate by -45 offset character 0, 0, 0 
set offset 0, 0, 0, 0
set xtics norangelimit 
set ytics nomirror
set termoption dashed
set grid ytics lt 0
set ylabel "Percentage of Instructions (Log Scale)"
plot "plot/spec-dist.csv" using 0:($2*100):(($2-$3)*100):(($2+$3)*100):xtic(1) title "SPECint2006" lc rgb 'black' lt 1 pt 6 ps .5 with yerrorbars, \
     "plot/babel-dist.csv" using 0:($2*100):xtic(1) title "Babel" lc rgb 'black' lt 1 pt 7 ps .2 with points, \
     "plot/babel-dist.csv" using 0:($3*100):xtic(1) notitle lc rgb 'black' lt 1 pt 7 ps .2 with points, \
     "plot/babel-dist.csv" using 0:($4*100):xtic(1) notitle lc rgb 'black' lt 1 pt 7 ps .2 with points, \
     "plot/babel-dist.csv" using 0:($5*100):xtic(1) notitle lc rgb 'black' lt 1 pt 7 ps .2 with points, \
     "plot/babel-dist.csv" using 0:($6*100):xtic(1) notitle lc rgb 'black' lt 1 pt 7 ps .2 with points




==> plot/plot-dist-logscale-cv <==
set term pdf size 6,3 font "Aerial,15"
set output "plot/dist-logscale-cv.pdf"
set size ratio 0.6
set yrange [0.01:100]
set xrange [-1:27]
set logscale y
set datafile separator ","
set xtics border out nomirror rotate by -45 
#set xtics border out scale 0,0 nomirror rotate by -45 offset character 0, 0, 0 
set offset 0, 0, 0, 0
set xtics norangelimit 
set ytics nomirror
set termoption dashed
set grid ytics lt 0
set ylabel "Percentage of Instructions (Log Scale)"
plot "plot/spec-dist.csv" using 0:($2*100):(($2-$3)*100):(($2+$3)*100):xtic(1) title "SPECint2006" lc rgb 'black' lt 1 pt 6 ps .5 with yerrorbars, \
     "plot/cv-dist.csv" using 0:($2*100):xtic(1) title "Code Virtualizer" lc rgb 'black' lt 1 pt 7 ps .2 with points, \
     "plot/cv-dist.csv" using 0:($3*100):xtic(1) notitle lc rgb 'black' lt 1 pt 7 ps .2 with points, \
     "plot/cv-dist.csv" using 0:($4*100):xtic(1) notitle lc rgb 'black' lt 1 pt 7 ps .2 with points, \
     "plot/cv-dist.csv" using 0:($5*100):xtic(1) notitle lc rgb 'black' lt 1 pt 7 ps .2 with points, \
     "plot/cv-dist.csv" using 0:($6*100):xtic(1) notitle lc rgb 'black' lt 1 pt 7 ps .2 with points




==> plot/plot-size <==
#set term post eps enhanced color
#set output "plot/size.eps"
set term pdf font "Aerial,15"
set output "plot/size.pdf"
set xrange [-10:50]
set yrange [0: 2500]
set xtics (0,10,20,30,40)
set format x "%g %%"
set datafile separator ","
set termoption dashed
set border 15
set datafile missing '-'
set key spacing 1.1 enhanced
set key bottom right
set key at 50,250
set key maxrows 3
set xtics nomirror
set ytics nomirror
set xlabel "Obfuscation Level"
set ylabel "Binary Size (KB)"
plot "plot/size-data.csv" using ($1*100):2 smooth unique lt 1 lc 7 lw 5 title "bzip2" with lines, \
     "plot/size-data.csv" using ($1*100):3 smooth unique lt 2 lc 7 title "mcf" with lines, \
     "plot/size-data.csv" using ($1*100):4 smooth unique lt 3 lc 7 title "regexp" with lines, \
     "plot/size-data.csv" using ($1*100):5 smooth unique lt 4 lc 7 title "svm_light" with lines, \
     "plot/size-data.csv" using ($1*100):6 smooth unique lt 1 lc 7 title "oftpd" with lines, \
     "plot/size-data.csv" using ($1*100):7 smooth unique lt 5 lc 7 title "mongoose" with lines



==> shortorlong.tex <==
\renewcommand{\shortlong}[2]{#1}


==> shortversion.tex <==
\renewcommand{\shortlong}[2]{#1}

